Impact of Community Structure on Cascades

We study cascades under the threshold model on sparse random graphs with community structure. In this model, individuals adopt the new behavior based on how many neighbors have already chosen it. Specifically, we consider the permanent adoption model wherein individuals that have adopted the new behavior (or opinion) cannot change their state. We present a differential-equation-based tight approximation to the stochastic process of adoption and prove the validity of the mean-field equations. In addition, we characterize both necessary and sufficient conditions for contagion to happen no matter how small the set of initial adopters is. Finally, we study the problem of optimum seeding given budget constraints and propose a gradient-based heuristic seeding strategy. Our algorithm, numerically, dispels commonly held beliefs in the literature that suggest the best seeding strategy is to seed over the vertices with the highest number of neighbors.

==> Sections/additional_Note.tex <==
 For ease of explanation, we assume the same degree distribution for the cross-community links but we believe that our results hold even if this weren't the case.

==> Sections/review.tex <==
The threshold model~\cite{Granovetter1978,Schelling1978,Naylor1990,Watts2007,Moore2014} is a well accepted model for explaining the adoption of a new technology, opinion or behavior in a population that interacts via a social network. The linear threshold model, where the threshold is a function of the degree, was analyzed for the contagion threshold for specific graphs in~\cite{Morris2000}, and using heuristically derived formulae for single community random graphs in~\cite{Watts2002,Lopez2008}. The results on the single community random graphs were rigorously proved using branching processes in~\cite{Lelarge2012}, where the importance of pivotal players (those whose degree is low enough that one neighbor will make them adopt the new behavior) was identified and studied. Similar results were derived using the differential equation method in~\cite{Balogh2007,Amini2010}, and in~\cite{Como2019} for the non-permanent adoption model.

The threshold model has been studied for networks with communities, but using heuristically derived mean-field approximations and approximate differential equations~\cite{Galstyan2007,Gleeson2007,Gleeson2008,Lopez2008,Galstyan2009}. In these studies, it was numerically shown in~\cite{Gleeson2008,Galstyan2007} for the linear threshold model that the community structure leads to a different dynamic in terms of the evolution of the cascade itself. It is important to note that the authors in these works postulate both the mean-field equation and the differential equations in an \emph{ad hoc} manner without a formal proof. This is particularly the case for the multi-community work in~\cite{Gleeson2008,Galstyan2007} where the authors combine the adoption processes in the different communities without a proper mathematical justification.

The problem of maximizing influence propagation in networks, by targeting certain influential vertices that have the potential to influence many others, has been an important follow-up problem~\cite{Granovetter1978,Schelling1978,Naylor1990,Watts2007} once the impact of a social network on behavior adoption was discovered.
%From the algorithmic standpoint, this selection problem can be stated as follows~\cite{Domingos:2001:MNV:502512.502525}: given a social network, an influence model (say the threshold model), and a set of vertices $S$, let $\sigma(S)$ be the expected number of vertices that will be activated by the end of the influence propagation process. Then, for a given budget $b$, the influence maximization problem is concerned with finding the set $S$ of size $b$ that maximizes the return $\sigma(S)$.
%The objective is to find the optimal subset of vertices with a pre-specified size to target initially so as to maximize the eventual influence propagation in the entire population.
While this problem is known to be NP hard for many influence models, several approximate methods have been designed, see e.g.,~\cite{Kempe2003,Mossel2010}.
% An important result established in~\cite{Kempe:2003:MSI:956750.956769,doi:10.1137/080714452} states that for a class of models, a simple greedy algorithm, which selects the next best candidate vertex, yields a solution that is guaranteed to be within $(1-1/e)$ of the optimal, under a few crucial assumptions.
%Although this result is general, it is very sensitive to some crucial assumptions. To be more specific, let us focus on the so called linear threshold models where a vertex $v$ is activated whenever the fraction of its active neighbors exceeds some predefined threshold $\theta_v$. In order to apply the results in~\cite{Kempe:2003:MSI:956750.956769,doi:10.1137/080714452}, we need to assume that $\theta_v$ are i.i.d. uniform in the interval $[0,1]$. In the Appendix~\ref{app:greed} we show by an example how these results break if $\theta_v$ is assumed to be fixed.
%
A contrasting strategy to identifying and targeting influential vertices is to use viral marketing~\cite{Schelling1978,Naylor1990,Vega2007}. % by seeding a new behavior in a population. %, i.e., targeting a certain fraction of the population.
%Often this can be network-structure agnostic, i.e., target a certain fraction of the population, but it can also use properties such as the degrees of the vertices, without the knowledge of the fine or local network structure, i.e., the location of the vertices.
A randomized version of viral marketing, also referred to as seeding or advertising in the paper, was studied in~\cite{Lelarge2012,Amini2010} where the resulting cascade was precisely identified. The results in~\cite{Lelarge2012} also suggested that targeting higher degree vertices is a better seeding strategy over degree-unaware random seeding. With community structure,~\cite{Gleeson2007,Gleeson2008,Galstyan2009} showed that the seeding strategies could be dramatically different from the one-community optimal strategies. Typically asymmetric seeding strategies, wherein the seeding is principally carried out in one community over another, were shown to perform better than more uniform (over the communities) seeding strategies. %For e.g.,~\cite{gleeson2008cascades} shows a four community example where seeding in community 1 produces a global cascade but seeding in community 4 doesn't. Again it should be emphasized that since the analysis of~\cite{gleeson2008cascades,galstyan2007cascading}  is not mathematically rigorous, the results can be questioned when not accompanied by large-scale simulations.







==> Sections/seeding.tex <==
A natural question to ask is ``what is the best seeding strategy given a budget constrain''. In this section, we formalize this question and provide a partial answer to that using a gradient based heuristic algorithm. By the analysis of Section \ref{sec:asymbhv}, we know we can always track the process upto points arbitrary close to $\bs{\mu}_*$, the closest fixed point of $\bs{F}$ to $\bs{1}$ in sup norm, where $\bs{F}$ is given by the right hand side of \eqref{eq:LMF-mu_jj} and \eqref{eq:LMF-mu_j-j}. We also know that if $\bs{\mu}_*$ is an stable equilibrium point then the process stops $\bs{\mu}_*$ with high probability. Now, using Corollary \eqref{cor:approx}, to give a partial answer to the question of optimum seeding, we will try to minimize $\Phi_1(\bs{\mu}_{*})+\Phi_2(\bs{\mu}_{*})$ by picking a seeding strategy $\bs{\alpha}$ that satisfies the budget constraint.

Assume the budget constraint is given in terms of the expected ratio of nodes that we can affect through advertisement. Mathematically, as $n\to\infty$, we can right the total budget constrain as follows:
\begin{align*}
\sum_{j,d_j,d_{-j}} \beta_j \, \p_{j,m}(d_j,d_{-j}) \, \alpha_{j}(d_j,d_{-j}) = \mathscr{B},
\end{align*}
where $\mathscr{B} > 0$ is a constant that denote the total available budget. Now, the optimization problem is given as follows:
\begin{align*}
\inf_{\bs{\alpha}} &&&\Phi_1(\bs{\bs{\alpha},\mu}_{*})+\Phi_2(\bs{\bs{\alpha},\mu}_{*})\\
\text{subject to} &&& \text{$(i)$ Budget constraint:}\sum_{j,d_j,d_{-j}} \beta_j \, \p_{j,m}(d_j,d_{-j}) \, \alpha_{j}(d_j,d_{-j}) = \mathscr{B},\\
&&& \text{$(ii)$ Definition of $\bs{\mu}_{*}$:}~ \bs{\mu}_* = \argmin_{\bs{u}: \bs{F}(\bs{\alpha},\bs{u}) = \bs{u}} \norm{\bs{u} - \bs{1}}_\infty,\\
&&& \text{$(ii)'$ Definition of $\bs{\mu}_{*}$:}~ \bs{\mu}_* = \lim_{s\to\infty}\bs{F}^s(\bs{\alpha},\bs{1}).
\end{align*}
By Corollary \ref{cor:F_Prop.Sol}, we know the conditions $(ii)$ and $(ii)'$ are equivalent. As the constraints are highly nonlinear, we take an easy heuristic approach to solve the above optimization problem.
